SocialCounterfactuals: Probing and Mitigating Intersectional Social Biases in Vision-Language Models with Counterfactual Examples

While vision-language models (VLMs) have achieved remarkable performance improvements recently, there is growing evidence that these models also posses harmful biases with respect to social attributes such as gender and race. Prior studies have primarily focused on probing such bias attributes individually while ignoring biases associated with intersections between social attributes. This could be due to the difficulty of collecting an exhaustive set of image-text pairs for various combinations of social attributes. To address this challenge, we employ text-to-image diffusion models to produce counterfactual examples for probing intersectional social biases at scale. Our approach utilizes Stable Diffusion with cross attention control to produce sets of counterfactual image-text pairs that are highly similar in their depiction of a subject (e.g., a given occupation) while differing only in their depiction of intersectional social attributes (e.g., race & gender). Through our over-generate-then-filter methodology, we produce SocialCounterfactuals, a high-quality dataset containing 171k image-text pairs for probing intersectional biases related to gender, race, and physical characteristics. We conduct extensive experiments to demonstrate the usefulness of our generated dataset for probing and mitigating intersectional social biases in state-of-the-art VLMs.

==> sections/8_ethical.tex <==
\section{Ethical Considerations}
\label{sec:ethical}

With the findings we present in this paper we aim to increase the understanding of bias in VLMs and probe mitigation strategies. We acknowledge that our work does not encompass all possible social attributes such as genders, races, occupations with the possibility of the selected categories also harboring stereotypes that cannot be assumed to represent their entire groups. On the lines of \cite{hall2023visogender} we understand we may often times miss intersectional characteristics that constitute a well accepted image of a person in a specific occupation or belonging to a race. We hope the techniques we present in this work can help reduce the various disparities and can be extended even further to include more genders, races, occupations and possibly other social characteristics. Only when we as a community continue to build on such guardrails can we increase the confidence in VLMs to make fair decisions that impact our lives. We understand that a mere use of a bias reduction strategy without deep understanding of various nuances does not guarantee a foolproof solution in bias elimination and still has scope to cause harm and stigmatize certain subsets of individuals. We hope this work can be built on and thoroughly studied before it's adoption to applications.

==> tables/tab-aggregate-metrics.tex <==
\begin{table}
    \centering
    \resizebox{1\textwidth}{!}{
    \begin{tabular}{l c c c c c c c}
        \toprule
        & & \multicolumn{3}{c}{\textbf{Text Retrieval}} & \multicolumn{3}{c}{\textbf{Image Retrieval}}  \\
        \cmidrule(lr){3-5}
        \cmidrule(lr){6-8}
        \textbf{HuggingFace Pre-trained Models} & \textbf{Evaluated Dataset} & \textbf{R@1} & \textbf{R@5} & \textbf{R@10} & \textbf{R@1} & \textbf{R@5} & \textbf{R@10} \\
        \midrule
        \multirow{2}{*}{bridgetower-large-itm-mlm-itc} & \cococfs & 21.72 (\textbf{-51\%}) & 46.94 (-35\%) & 58.65 (-29\%) & 17.93 (-47\%) & 38.94 (-35\%)& 49.95 (-30\%) \\
         & human-evaluated \cococfs  & 26.36 (\textbf{-41\%}) & 54.1 (-25\%) & 66.13 (-20\%) & 21.44 (-37\%) & 45 (-25\%) & 56.39 (-21\%) \\
        \midrule
        \multirow{2}{*}{flava-full} & \cococfs & 21.28 (\textbf{-57\%}) & 46.64 (-41\%) & 58.87 (-34\%) & 37.76 (-16\%) & 66.15 (-12\%)& 75.83 (-10\%) \\
         & human-evaluated \cococfs  & 26.1 (\textbf{-47\%}) & 54.23 (-31\%) & 66.83 (-25\%) & 43.4 (-3\%) & 72.35 (-3\%) & 81.44 (-4\%) \\
        \bottomrule
    \end{tabular}}
    \vspace{1mm}
    \caption{}
    \label{tab:aggregate-metrics}
\end{table}
